The Universal Arrow of Time I: Classical mechanics

Statistical physics cannot explain why a thermodynamic arrow of time exists, unless one postulates very special and unnatural initial conditions. Yet, we argue that statistical physics can explain why the thermodynamic arrow of time is universal, i.e., why the arrow points in the same direction everywhere. Namely, if two subsystems have opposite arrow-directions at a particular time, the interaction between them makes the configuration statistically unstable and causes a decay towards a system with a universal direction of the arrow of time. We present general qualitative arguments for that claim and support them by a detailed analysis of a toy model based on the baker's map.

==> ftslru.tex <==
%\maketitle

\pagestyle{empty}
\thispagestyle{empty}
%\documentstyle[12pt,twoside]{article}
%\pagestyle {empty}
%\begin{document}
%\renewcommand{\baselinestretch}{1}
\centerline{\large\bf } \vspace{0.2cm} \centerline{\large\bf }
\vspace{2.5cm} \centerline{\Large\bf  Универсальная стрела времени
I: Классическая механика  } \vspace{2.0cm} \centerline{Олег
Юрьевич Купервассер$^1$, Hrvoje Nikolic$^2$, Vinko Zlatic$^3$ }
\vspace{0.7cm} \centerline{\bf } \vspace{0.4cm} \centerline{\em
$^1$ Moscow State University, Scientific Research Computer Center
} \centerline{\em Moscow, Russia, $^1$ Email: olegkup@yahoo.com}
\centerline{\em $^{2,3}$ Theoretical Physics Division, Rudjer
Boskovic Institute} \centerline{\em  P.O.B. 180, HR-10002 Zagreb,
Croatia} \centerline{\em $^2$ Email: hrvoje@thphys.irb.hr, $^3$
Email: Vinko.Zlatic@irb.hr}
\par
\vspace{2.0cm}


$$    $$
$$    $$
$$    $$
$$    $$
\centerline{\em Август 2011}
\par
\vspace{0.8cm}
%\renewcommand{\baselinestretch}{1.9}
\newpage
%\end{document}


==> univTAfp_rus.tex <==


\begin{abstract}
Статистическая физика не может объяснить, почему термодинамическая
стрела времени существует, если не постулируются очень специальные
и неестественные начальные условия. Однако, мы утверждаем, что
статистическая физика может объяснить, почему термодинамическая
стрела времени универсальна, то есть, почему стрела времени
направлена в одинаковом направлении повсюду. А именно, если у двух
подсистем есть противоположные направления стрелы времени
первоначально, взаимодействие между ними делает конфигурацию
статистически неустойчивой и вызывает переход к системе с
универсальным направлением стрелы времени. Мы даем общие
качественные аргументы в пользу такого взгляда и иллюстрируем их
детальным анализом "игрушечной" модели, основанной на
"Преобразовании Пекаря".
\end{abstract}

\vspace*{0.5cm}
PACS: 05.20.-y, 05.45.-a
%05.20.-y  Classical statistical mechanics
%05.45.-a  Nonlinear dynamics and chaos

Keywords: стрела времени, увеличение энтропии, преобразование Печника



\section{Введение}

Происхождение стрелы времени - одна из самых больших нерешенных
загадок в физике
\cite{reichenbach,davies,penrose,price,zeh}. Хорошо
установлено, что большинство стрел времени может быть приведено к
термодинамической стреле, но происхождение термодинамической
стрелы времени остается тайной. А именно, существование
термодинамической стрелы времени означает, что система не
находится в состоянии с максимально возможной энтропией. Но это
означает, что система не находится в самом вероятном состоянии,
что не имеет никакого статистического объяснения. Факт увеличения
энтропии со временем означает, что система была в даже менее
вероятном состоянии в прошлом, что делает задачу еще более
сложной. Конечно, рост энтропии  со временем может быть описан,
при предположении, что Вселенная была в состоянии с очень низкой
энтропией вначале. Однако при этом никак нельзя объяснить, почему
Вселенная началась с такого очень специального и неестественного
начального условия.

В недавней статье Maccone \cite{mac} утверждал, что задача
происхождения стрелы времени может быть решена квантовой
механикой. Он показал, что в квантовой механике все явления,
которые оставляют след в памяти наблюдателя (и, следовательно,
могут быть изучены физикой) являются именно теми, при которых
энтропия увеличивается. (Следует отметить, что аргумент о стирании
памяти наблюдателя при убывании энтропии и соответствующие
мысленные эксперименты, рассмотренные в \cite{mac}
использовалась и в более ранних работах других авторов для
разрешения парадокса роста энтропии и квантового парадокса
редукции волнового пакета
\cite{vaidman,kuper04,kuper05}.) ]). Из этого Maccone
заключает, что таким образом второй закон термодинамики сводится к
простой тавтологии, автоматически решая проблему стрелы времени в
физике. Однако, некоторые слабости аргументов, используемых
Maccone в \cite{mac} указаны в статьях
\cite{com1,com2,com3}. Как ответ на одно из этих
возражений, в более поздней публикации \cite{mac2} сам Maccone
понял, что его подход полностью не решает проблему происхождения
стрелы времени, потому что квантовый механизм также требует крайне
невероятных начальных условий, которые не могут быть объяснены,
исходя из его аргументов.

Все же, как и Maccone в  \cite{mac2}, мы полагаем, что
некоторые идеи, представленные в  \cite{mac} и \cite{mac2}
действительно помогают лучше понять проблему стрелы времени. Цель
этой статьи состоит в том, чтобы далее разработать, улучшить,
разъяснить, и расширить некоторые из идей, которые были
представлены в \cite{mac,mac2,com2},  и также в несколько
отличном контексте в
\cite{kuper04,kuper05,zeh1,zeh2,kupervasser-big,thomson,Leb}.
В частности, в отличие от Maccone в  \cite{mac,mac2}, мы
утверждаем, что квантовая механика не является существенным
фактором для разрешения этой проблемы. Поэтому в этой статье мы
рассматриваем только классическую статистическую физику.

Идея разрешения этого парадокса следующая. Даже при том, что
статистическая физика не может объяснить, почему термодинамическая
стрела времени существует, по крайней мере, становится возможным
объяснить, почему термодинамическая стрела времени универсальна.
То есть, мы можем объяснить, почему стрела указывает в одинаковом
направлении повсюду. А именно, если у двух подсистем есть
противоположные направления стрелы времени первоначально,
взаимодействие между ними делает конфигурацию статистически
неустойчивой и вызывает переход к системе с универсальным
направлением стрелы времени. Это, конечно, полностью не решает
проблему происхождения стрелы времени. Но, по крайней мере,
облегчает её решение.

Статья организована следующим образом. В следующем разделе мы
представляем свои главные идеи в интуитивной нетехнической форме.
После этого, в разделе~\ref{SEC3Rus} мы изучаем статистические
свойства "Преобразования Пекаря" (некоторые основные свойства
которого представлены в Приложении), которое служит "игрушечной"
моделью для того, чтобы изучить характерные особенности обратимых
хаотических Гамильтоновых систем. Как побочный результат, в этом
разделе мы также проясняем разницу между различными определениями
понятия "энтропии". Затем, в разделе~\ref{SEC4Rus} мы изучаем
эффекты слабых взаимодействий между подсистемами, которые, без
взаимодействия, эволюционируют согласно "Преобразованию Пекаря". В
частности мы объясняем, как слабые взаимодействия разрушают
противоположные стрелы времени подсистем, делая их намного менее
вероятными, чем в случае без взаимодействия. Наконец, в
разделе~\ref{SEC5Rus} мы даем качественное обсуждение наших
результатов, включая их совместимость с наличием
сильновзаимодействующих систем, в которых энтропия подсистемы
может уменьшиться со временем.


\section{Главные идеи.}
\label{SEC2Rus}

Чтобы избегать двусмысленности в дальнейших обсуждениях, позвольте нам сначала объяснять наши основные понятия и терминологию, используемую в остальной части статьи. Для той цели полезно изобразить время как непрерывную 1-мерную линию. Линия параметризуется непрерывным параметром $t$. Такая параметризация обязательно создает ориентацию линии времени с направлением, указывающим от меньших к большим величинам $t$. Мы можем использовать эту ориентацию, чтобы определить понятия типа "прежде" и "после", "прошлое" и "будущее", или "начальный" и "заключительный". В этой статье, если не заявлено иначе, под этими понятиями мы подразумеваем понятия, определенные относительно этой временой координаты $t$. Однако, мы подчеркиваем, что такая ориентация времени координаты - просто вопрос выбора и не имеет никакого физического содержания. В частности, такая ориентация сама по себе {\em не} создает стрелу времени. Вместо этого, под стрелой времени мы подразумеваем {\em физическое} явление, как, например, увеличение  или уменьшение энтропии со временем $t$. Когда стрела времени в одном и том же направлении всюду на линии времени, тогда временная координата может быть определена так, что ориентация $t$ совпадает со стрелой времени. Это позволяет нам злоупотреблять языком в некоторых местах, утверждая, что энтропия "увеличения", а не "уменьшения" со временем, но нужно иметь в виду это, различие между увеличением и уменьшением со временем - просто вопрос определения. Вообще же, стрела времени и ориентации $t$ - логически независимые понятия.

Теперь позвольте нам обсудить термодинамическую стрелу времени.
{\it Априорно}, вероятность наличия термодинамической стрелы
времени очень низка. Однако идея состоит в том, чтобы думать в
терминах условных вероятностей. Учитывая, что термодинамическая
стрелка существует, что может мы, используя статистические
аргументы, вывести из этого?

Чтобы ответить на этот вопрос, позвольте нам начать с законов
микроскопической теории. Мы предполагаем, что динамика
микроскопических степеней свободы описана набором дифференциальных
уравнений второго порядка (с производными по времени), которые
являются инвариантными при обращении времени  $t\rightarrow -t$.
Таким образом, у обоих направлений времени есть априорно равные
роли. Чтобы определить единственное решение уравнений динамики
движения, также нужно выбрать некоторое "начальное" время  $t_0$ ,
на котором должны быть определены начальные условия. ("Начальное"
время не обязательно должно быть самым ранним временем, в которое
Вселенная вошла в существование. Для любого  $t_0$ , в котором
определены начальные условия, уравнения динамики движения
единственным образом определяют состояние Вселенной как для
$t>t_0$ , так и для  $t<t_0$). Это - просто обычный специфический
момент времени, который может быть взят даже в "будущем".
Действительно, в этой статье мы принимаем картину "блочной
Вселенной"  (смотри, например,
\cite{price,ellis,nik1,nik2} и ссылки там), согласно
которой время не "течет". Вместо этого Вселенная - это просто
"статический" объект в 4-ёх пространственно-временных измерениях.

Конечно, {\it априорная} вероятность небольшой энтропии в момент
$t_0$ очень низка. Но при условии, что энтропия, {\em данная в
момент} $t_0$, является небольшой, какова вероятность, что
существует термодинамическая стрела времени? Она, конечно, очень
высока. Однако, полагая, что энтропия в $t_0$ низка, самый
вероятный выбор состоит в том, что энтропия увеличивается в {\em
обоих} направлениях с минимумом в $t_0$. (Мы представляем пример на Рис. ~\ref {figintsym} Разлела ~\ref {SECnumsim}.) Ясно, в таком случае система является симметричной при  инверсии $(t-t_0) \rightarrow - (t-t_0)$. Термодинамическая стрела времени для $t> t_0$ имеет противоположное направление, чем для $t <t_0$. Таким образом, даже при том, что никакое направление времени не является привилегированным {\em глобально}, термодинамическая стрела времени может, тем не менее, задаваться {\em в местном масштабе} для  различных моментов времени $t \neq t_0$.

С другой стороны, в те моменты времени,  на которых мы делаем измерение на практике, энтропия действительно низка, но энтропия не увеличивается в обоих направлениях. Вместо этого, это она увеличивается в только одном направлении. (Другими словами, типичное время $t_0$, в которое мы делаем измерение - это не момент времени, в которое энтропия достигает минимума. Это является причиной, что мы не наблюдаем временню симметрию) Для  типичного момента $t_0$, не только "начальная" энтропия определена, но и специфическоенаправление увеличения энтропии определено также. На микроскопическом уровне, это связано с фактом, что в момент $t_0$ мы  должен определить не только начальные положения частиц, но также и их начальные скорости.

А теперь центральный вопрос этого раздела. Учитывая, что в момент
времени  $t_0$ энтропия низка, почему энтропия в увеличивается в
этот момент $t_0$ в одном и том же направлении (принимаемом за
положительное) повсюду? Казалось бы, более вероятно, что
направление  увеличения энтропии изменяется от точки в момент
$t_0$? Если так, тогда почему мы не наблюдаем это? Другими
словами, почему стрела времени {\em универсальна}, имея одно и том
же направление повсюду для данного момента $t_0$? Мы назовём эту
проблему  проблемой {\em универсальности стрелы времени}.

В этой статье мы утверждаем, что {\em эта} задача может быть
решена статистической физикой. Короче говоря, наше решение
следующие. Если мы игнорируем взаимодействия между различными
подсистемами, то, при условии, что в  $t_0$ энтропия низка, то
самый вероятный выбор, действительно, что направление стрелы
времени изменяется от точки к точке. С другой стороны, если
различные подсистемы взаимодействуют друг c другом, то это больше
не самый вероятный выбор. Вместо этого, даже если направление
стрелки времени изменяется от точки к точке в момент $t_0$, то
взаимодействие обеспечивает естественный механизм, который
выравнивает все стрелы времени в одном и том же направлении.

Чтобы проиллюстрировать парадокс стрелы времени, часто
используются мысленные эксперименты  Лошмидта (парадокс обращения
времени) и Пуанкаре (теорема о возвратах). Соответствующие
парадоксы в классической механике решены следующим образом.
Классическая механика позволяет, по крайней мере в принципе,
исключить любой эффект влияния наблюдателя на наблюдаемую систему.
Однако, большинство реальных систем являются  {\em хаотическими}.
Таким образом, даже слабое возмущение может привести к
экспоненциальному расхождению траекторий. Кроме того, существует
незначительное взаимодействие между наблюдателем и наблюдаемой
системой. Как простой пример, рассмотрим газ, расширяющийся из
небольшой области пространства в большой объем. В этом процессе,
идущем с увеличением энтропии, изменение во времени
макроскопических параметров устойчиво по отношению к небольшим
внешним возмущениям. С другой стороны, если все скорости будут
обращены, то газ сожмется в начальный небольшой объем, но только в
отсутствие любых возмущений. Этот  процесс с уменьшением энтропии
очевидно неустойчив, и небольшое внешнее возмущение преобразовало
его в процесс с ростом энтропии. Таким образом, процессы с
увеличением энтропии, устойчивы, а с уменьшением - нет.
Естественное следствие этого - то, что направление стрелы времени
(которое определено  ростом энтропии) как наблюдателя, так и
наблюдаемой системы выравнивается к одному и тому же направлению,
из-за неизбежного незначительного взаимодействия между ними. Они
могут возвратиться назад к начальному состоянию как в парадоксе
Лошмидта, так  и в парадоксе Пуанкаре только вместе (как система в
целом). Таким образом, память наблюдателя оказывается стертой в
конце, потому что мы предполагаем, что все, включая мозг наблюдателя, полностью вернулось к состоянию, идентичному прежнему состоянию, описывающему систему прежде, чем память была создана.. В  процессе 
этого возврата стрелы времени как наблюдателя, так и наблюдаемой
системы указывают в направлении обратном первоначальному. Отсюда
можно вывести два следствия. Во-первых, рост энтропии наблюдается
как в целой системе, так и в ее двух частях относительно
собственной стрелы времени наблюдателя, несмотря на то, что
энтропия уменьшается в координатном времени. Во-вторых, память
наблюдателя стерта не только в самом конце, но также уже и близко
к конечной точке, потому что наблюдатель не помнит своего
"прошлого" (определенного относительно координатного времени), но
помнит своё "будущее". Конечно, сам наблюдатель не может знать, что стрела времени полностью изменила ее направление, потому что он может только наблюдать {\em физическое} "прошлое" и  "будущее" определенное не относительно координатного времени, а относительно направления, в котором энтропия увеличивается.


Действительно, может казаться весьма вероятным, что взаимодействие
выровняет все стрелы времени в одном и том же направлении. Но тут
возникает вопрос, - в каком именно направлении из двух возможных?
Как может какое-нибудь одно направление быть предпочтительным,
когда оба направления  {\it априорно} одинаково вероятны? Общее
направление выбирается случайно или оно может быть эффективно
предсказано? Если есть две подсистемы с противоположными
направлениями времени в  $t_0$, то совместная система выберет
направление "более сильной" подсистемы как их общее направление.
Но какая подсистема будет "более сильная"? Та ли, что обладает
большим числом степеней свободы? Или она выбирается по иному
принципу?

На самом деле, "более сильная" стрела времени - это та, которая
сонаправлена с координатным направлением времени. Действительно,
ситуация тут не симметричная. Для $t<t_0$ (когда стрелы времени
противонаправлены) взаимодействие отсутствует, а для $t>t_0$ оно
появляется. Это асимметрия взаимодействия и определяет наблюдаемую
асимметрию времени.

Обратим внимание также, что механизм, изложенный выше, не зависит значительно от относительных размеров этих двух подсистем. В частности если они имеют равный размер, то есть, для одной половины системы стрела времени ориентирована противоположно другой половине для $t_0 <t \leq t_1$, общая стрелка времени для $t> t_1$ будет все еще определяться вышеупомянутой асимметрией в знании.



Далее обратим внимание, что качественные вероятностные аргументы, изложенные выше, верны для большинства систем, но не обязательно для всех возможных системах. Действительно, есть интересные физические системы, типа спин-эхо, в которых подсистема может иметь стрелу времени противоположную стреле времени окружающей ее среды. Дело в том, что такие системы - исключения, а не правило. Таким образом, наши качественные вероятностные аргументы, несмотря на наличие  таких систем все еще верны, при условии, что они не рассматриваются как строгие законы без исключений.


 
Фактически, не трудно понять качественно, почему исключения типа спин-эха существуют. Во-первых, это  система с относительно небольшим количеством степеней свободы, что делает статистические аргументы менее точными и флюктуации более вероятны в таких случаях. Во- вторых, взаимодействие этой системы с окружающей средой настолько слабо, что механизм выравнивания направления роста энтропии берет больше времени, чем в большинстве других систем. Действительно, даже система спин-эха,  в конечном счете, после достаточного времени, выравнивает направление стрелы времени с ее окружающей средой. 


Поскольку никакое направление времени не является {\it априорно} привилегированным, позвольте нам также кратко обсудить ситуацию, инверсную к вышеупомянутой. Для этой цели, теперь позвольте нам предположить, что взаимодействие существует только для $t <t _ {-1} $, где $t _ {-1} <t_0$. С помощью полностью аналогичных рассуждений, теперь мы можем заключить, что энтропия увеличится в {\em отрицательный} направление времени для $t <t _ {-1} $. 

Полностью симметрический вариант также возможен. Положим, что взаимодействие существует и для $t> t_1$, и для $t <t _ {-1} $ (но не для $t _ {-1} \leq t \leq t_1$). В этом случае, энтропия увеличивается в {\em положительным} направлении времени для $t> t_1$ {\em и} в {\em отрицательном} направлении времени для $t <t _ {-1} $. Другими словами, подобно к случаю на Рис. ~\ref {figintsym} Раздела ~\ref {SECnumsim}, энтропия увеличится в {\em обоих} направлениях, но в  различные моменты времени.

Одно дополнительное примечание относительно начальных условий. Даже когда две подсистемы имеют противоположные направления термодинамической стрели времени, мы выбираем начальные условия для них обоих в {\em один тот же} момент времени $t_0$, скажем в прошлом. Действительно, выбор, для которого $t_0$ находится в прошлом - естественный выбор для подсистемы, в которой энтропия увеличивается со временем. Однако, этот выбор не настолько естественен для другой подсистемы, в которой энтропия уменьшается со временем. Для такой подсистемы было бы более естественно выбрать "начальное" условие в будущем. Или более широко, можно было бы изучить много подсистем, каждую с начальными условиями в разнментые моменты времени. Подчеркнем, что в этой статье мы не изучаем такие более общие начальные условия, потому что, когда взаимодействия между подсистемами существует, начальные условия, выбранные в разные моменты времни для разных подсистем, не могут быть заданы произвольно. А именно, для таких начальных условий, заданных в разные моменты времени, последовательное решение динамических уравнений движения не может даже существовать. И даже когда такое решение существует,  не известно, как доказать его существование или как найти это решение в численной форме.


Теперь мы можем понять, почему стрела времени универсальна. Пусть
есть подсистема, у которой есть стрела времени направленная
противоположно нашей общей стреле времени, и эта подсистема или
наблюдается, или не наблюдается нами. Если она не наблюдается, то
это не нарушает того факта, что наша стрела времени кажется
универсальной нам. Если она наблюдается, тогда она взаимодействует
с нами. А это взаимодействие приводит к тому, что эти стрелы
времени не могут быть противоположными в течение долгого времени.
В любом случае  - {\em то, что  мы наблюдаем, должно иметь то же
самое направление времени} (, что и наше (кроме, возможно, очень
короткого временного интервала). Это подобно рассуждению в
\cite{mac}, с той важной разностью, что наше рассуждение не
базируется на квантовой механике.

В остающихся разделах мы подтверждаем эти интуитивные идеи более
количественным анализом.




\section{Статистическая физика Преобразования Пекаря}
\label{SEC3Rus}

Преобразования Пекаря (для более детального анализа смотри
Приложение  \ref{app1Rus}) отображает любую точку единичного
квадрата на другую точку того же самого квадрата. Мы изучаем набор
$N>>1$ таких точек (называемых "частицами"),  который движется под
воздействием Преобразования Пекаря. Это является "игрушечной"
моделью для "газа", который обладает всеми типичными свойствами
классических Гамильтоновых обратимых детерминированных хаотических
систем. Действительно, из-за его простоты, Преобразования Пекаря
широко используется в таких целях
\cite{prigogine1,elskens,gaspard,hartmann}.

\subsection{Макроскопическая энтропия и энтропия ансамбля}

Чтобы определить удобный набор макроскопических переменных, мы
делим единичный квадрат на 4-ре равных подквадрата. Пусть  4-ре
переменных  $N_1$, $N_2$, $N_3$, $N_4$, обозначают число "частиц"
в соответствующих подквадратах. Они  и являются макроскопическими
переменными для нашей системы. (Есть, конечно, много других
удобных способов определить макроскопические переменные, но общие
статистические закономерности не должны зависеть от этого выбора).
 {\em Макроскопическая энтропия} $S_{\rm m}$ данного макросостояния
  определяется числом различных микросостояний, соответствующих этому
  макросостоянию, и описывается следующей формулой
\begin{equation}\label{macrentRus}
 S_{\rm m}=-N\sum_{k=1}^{4} \frac{N_k}{N} \, {\rm log} \left( \frac{N_k}{N} \right)
=- \sum_{k=1}^{4} N_k \, {\rm log} \left( \frac{N_k}{N} \right) .
\end{equation}
Эта энтропия максимальна, когда распределение частиц равномерно,
когда  $S_{\rm m}$ равна $S_{\rm m}^{\rm max}=N \, {\rm log} 4$. .
В то время энтропия минимальна, когда все частицы находятся в
одном подквадрате, т.е. когда  $S_{\rm m}=0$.

Пусть  $(x,y)$ dобозначают координаты точки на единичном квадрате.
На физическом языке это соответствует положению частицы в 2-мерном
фазовом пространстве. Для  $N$ частиц мы рассматриваем
статистический ансамбль с плотностью вероятности $\rho(x_1,y_1;
\ldots ;x_N,y_N;t)$ на $2N$ размерное фазовое пространство. Здесь
$t$ i- временной параметр, который имеет  дискретные значения
$t=0,1,2,\ldots$ fдля Преобразования Пекаря. Тогда  {\em энтропия
ансамбля } определяется как
\begin{equation}
 S_{\rm e}=-\int \rho(x_1,y_1; \ldots ;x_N,y_N;t) \; \log \rho(x_1,y_1; \ldots ;x_N,y_N;t) \, dX ,
\end{equation}
где
\begin{equation}
 dX \equiv dx_1 \, dy_1 \, \cdots dx_N \, dy_N.
\end{equation}
В общем случае, $\rho$ и $S_{\rm e}$ изменяются в процессе
эволюции, определяемой Преобразованием Пекаря, и зависят от
начальной  $\rho$. Однако, если начальная функция плотности
вероятности имеет форму
\begin{equation}
 \rho(x_1,y_1; \ldots ;x_N,y_N) = \rho(x_1,y_1) \cdots \rho(x_N,y_N) ,
\end{equation}
которая соответствует некоррелированной функции плотности, тогда
функция плотности вероятности остается некоррелированной в
процессе дальнейшей эволюции.

Так, например, рассмотрим функцию  $\rho(x_l,y_l)$, которая
равномерна в пределах некоторой подобласти  $\Sigma$ (с площадью
$A<1$) единичного квадрата, и обращается в нуль за пределами
$\Sigma$. Другими словами, пусть
\begin{equation}
 \rho(x_l,y_l,t)=
\left\{
\begin{array}{l}
\displaystyle
1/A \;\;\;\; {\rm for} \; (x_l,y_l) \;  {\rm inside}\; \Sigma, \\
\displaystyle
0  \;\;\;\; {\rm for} \; (x_l,y_l) \;  {\rm outside}\; \Sigma .
\end{array}
\right.
\end{equation}
В этом случае
\begin{equation}
 S_{\rm e}=-\left(\frac{1}{A}\right)^N  {\rm log} \left(\frac{1}{A}\right)^N  A^N
= N \, {\rm log} A.
\end{equation}
Так как  $A$ dA не изменяется в процессе эволюции, определяемой
Преобразованием Пекаря, то и $S_{\rm e}$ является постоянной в
процессе эволюции, определяемой Преобразованием Пекаря. Этот
пример иллюстрирует, что $S_{\rm e}$ является фактически
постоянной для  {\em произвольной}  начальной функции. Для
доказательства, позвольте нам разделить единичный $2N$-мерный ящик
на большое количество небольших областей  $\Sigma_a$, для каждой
из которых вероятность равна $\rho_a$В процессе эволюции каждая
область $\Sigma_a$ изменяет форму, но ее  $2N$-мерная "площадь"
$A_a$ остается неизменной. Кроме того, вероятность  $\rho_a$ на
новой области $\Sigma_a$ также остается неизменной. Следовательно,
энтропия ансамбля  $S_{\rm e}=-\sum_a  A_a^N \rho_a \, {\rm
log}\rho_a$ остается неизменной также. Это - основная идея
дискретной версии доказательства, но и непрерывная версия может
быть сделана подобным же способом.


\subsection{Соответствующие и несоответствующие макроскопические переменные}

Макроскопические переменные, определенные в предыдущем подразделе
имеют следующие свойства:
\begin{enumerate}
 \item Для большинства начальных микросостояний, имеющих свойство  $S_{\rm m}<S_{\rm m}^{\rm max}$,
$S_{\rm m}$ увеличивается под действием Преобразования Пекаря.
 \item Для большинства начальных микросостояний, имеющих свойство  $S_{\rm m}=S_{\rm m}^{\rm max}$,
$S_{\rm m}$ остается постоянной под действием Преобразования
Пекаря.
 \item Два, описанных ыше свойства  остаются в силе, когда Преобразования Пекаря дополнено небольшим шумом.
\end{enumerate}
Назовем макропеременные, имеющие эти свойства, подходящими
макропеременными. (Они являются "подходящими" в смысле, что соответствующий макроскопический закон увеличения энтропии может быть получен только, когда макропеременные повинуются этим свойствам.)

Отнюдь не любой разумный выбор макропеременных является
подходящим. Это можно проиллюстрировать примером. Разделим
единичный  квадрат на   $2^M$ одинаковых вертикальных полос
($M \gg 1$)). Мы определяем новое множество макропеременных как
номера частиц в каждой из этих полос. Подобно формуле
(\ref{macrentRus}), соответствующая макроскопическая энтропия
\begin{equation}\label{macrent2Rus}
 S_{\rm m}=- \sum_{k=1}^{2^M} N_k \, {\rm log} \left( \frac{N_k}{N} \right) ,
\end{equation}
где $N_k$ - число частиц в полосе  $k$. Выберем следующее
начальное условие: газ равномерно распределен в нечетных
вертикальных полосах, в то время как четные полосы пусты. Тогда
для этого начального условия выполняется  $S_{\rm m}<S_{\rm
m}^{\rm max}$ . При этом, в течение долгого времени эволюции
системы, осуществляемой в соответствии с Преобразованием Пекаря,
$S_{\rm m}$ не увеличивается ни для какого начального
микросостояния, соответствующего этому начальному макросостоянию .
В течение этой эволюции число заполненных полос уменьшается, а и
их толщина увеличивается, пока только одна толстая заполненная
вертикальная полоса не остается. Только после того, как это
произойдет,  $S_{\rm m}$ начинает увеличиваться. Следует обратить
внимание, что эволюция по направлению к единственной полосе может
быть легко разрушена небольшим возмущением.

Таким образом, мы видим, что вертикальные полосы приводят к
неподходящим макропеременным. В противоположность этому,
горизонтальные полосы приводят к подходящим макропеременным.
(Однако, макропеременные, использованные в  (\ref{macrentRus}),
все же более сподходящие, потому что они приводят к намного более
быстрому росту $S_{\rm m}$.) Эта асимметрия между вертикальными  и
горизонтальными полосами - следствие характерной асимметрии самого
Преобразования Пекаря относительно вертикальной и горизонтальной
координаты. Эта асимметрия подобна асимметрии между каноническими
координатами и импульсами в Гамильтоне классической механики для
многих реальных систем. А именно, для реальных систем гамильтоновы
функции  содержат только локальное взаимодействие между частицами,
где локальность подразумевает близость по координате, а не по
импульсу.

 Наконец,  обратим внимание, что эволюция макроскопических переменных  $N_k(t)$, $k=1,2,3,4$,
, найходится усреднением по ансамблю следующим образом
\begin{equation}
 N_k(t)=\int N_k(x_1,y_1; \ldots ;x_N,y_N;t)    \rho(x_1,y_1; \ldots ;x_N,y_N;t)  \, dX .
\end{equation}


\subsection{Огрубление}
\label{SECcoarsRus}

Как мы уже сказали, энтропия ансамбля (в отличие от
макроскопической энтропии) - всегда константа в течение эволюциии,
определяемой Преобразованием Пекаря. Однако, хотелось бы иметь
модифицированное определение энтропии ансамбля, при котором
энтропия увеличивалась бы подобно к макроскопической энтропии.
Такая модификация обеспечивается  {\em огрублением}, которое может
быть обеспечено введением огрубленной фазовой функции плотности
вероятности.
\begin{eqnarray}
\rho^{\rm coar}(x_1,y_1; \ldots ;x_N,y_N) & = &
\int \Delta(x_1-x'_1,y_1-y'_1; \ldots ;x_N-x'_N,y_N-y'_N)
\nonumber \\
& & \times \, \rho(x'_1,y'_1; \ldots ;x'_N,y'_N) \, dX' ,
\end{eqnarray}
 где $\Delta$ отлична от  нуля в некоторой области
$X'=0,0;\ldots ;0,0$. Таким образом, огрубленная энтропия ансамбля
\begin{equation}
 S_{\rm e}^{\rm coar}=-\int \rho^{\rm coar}(x_1,y_1; \ldots ;x_N,y_N) \;
\log \rho^{\rm coar}(x_1,y_1; \ldots ;x_N,y_N) \, dX .
\end{equation}
Конечно, функция $\Delta$ может быть выбрана многими способами.
Дадим теперь несколько примеров.

Первый пример - огрубление Больцмана , определяемое следующим
образом
\begin{equation}
\rho^{\rm coar}(x_1,y_1; \ldots ;x_N,y_N) = \rho(x_1,y_1) \cdots \rho(x_N,y_N) ,
\end{equation}
где
\begin{equation}
 \rho(x_1,y_1) = \int \rho(x_1,y_1; \ldots ;x_N,y_N) \,
dx_2 \, dy_2 \, \cdots dx_N \, dy_N ,
\end{equation}
И аналогично для других  $\rho(x_l,y_l)$.

Другой пример - изотропическое огрубление имеющее форму
\begin{eqnarray}
& \Delta(x_1-x'_1,y_1-y'_1; \ldots ;x_N-x'_N,y_N-y'_N) = &
\nonumber \\
& \Delta(x_1-x'_1) \Delta(y_1-y'_1) \cdots \Delta(x_N-x'_N) \Delta(y_N-y'_N) . &
\end{eqnarray}

Еще один пример - огрубление Пригожина  \cite{prigogine1}
\begin{equation}
\Delta(x_1-x'_1,y_1-y'_1; \ldots ;x_N-x'_N,y_N-y'_N) =
\Delta(y_1-y'_1)  \cdots  \Delta(y_N-y'_N) ,
\end{equation}
которое является анизотропным огрублением вдоль сжимыющего
направления  $y$.

Наконец, позвольте нам упоминать огрубление, основанное на
разделении системы на две меньшие взаимодействующие подсистемы.
Огрубленная энтропия ансамбля для полной системы определена как
арифметическая сумма неогрубленных энтропий ансамбля этих его
подсистем. Такая огрубленная энтропия игнорирует корреляции между
подсистемами.

Все эти типы огрубление имеют следующее свойство: Если начальное
микросостояние таково, что макроскопическая энтропия
увеличивается, то огрубленная энтропия ансамбля также будет
увеличиваться для этого начального микросостояния. При этом,
огрубление Пригожина  имеет следующие преимущества перед
огрублением Больцмана и изотропным огрублением:

Во-первых, если взять распределение начальных микросостояний
такое, что его макроскопическия энтропия уменьшается. Тогда
энтропия соответствующего ансамбля, огрубленная по Пригожину не
уменьшается. В то же время, энтропия ансамбля, огрубленная по
Больцману или согласно изотропному огрублению, будет уменьшаться.

Во вторых, предположим, что задано распределение начальных
микросостояний такое, что его макроскопическая энтропия
увеличивается. Теперь рассмотрим некоторое "заключительное"
состояние (называемое далее исходный ансамбль)  с большой
макроскопической энтропией, близкой к максимальной. После
достижения системой этого заключительного состояния, рассмотрим
полученное из него новое инверсное состояние, имеющего обратную во
времени эволюцию (Это достигается просто симметричным
пребразованием относительно диагонали единичного квадрата с
переменой местами координат x и y). Тогда энтропия ансамбля,
полученного после такого "обращения" и  огрубленная по Пригожину,
скачком уменьшается (по отношению к огрубленной энтропии
"необращенного" исходного ансамбля, из которого она получена этим
"обращением"). В то же время, энтропия ансамбля, огрубленная по
Больцману или изотропному огрублению, остаётся почти неизменной.

Таким образом, огрубление Пригожина обеспечивает, самое адекватное
описание закона увеличения энтропии ансамбля без всяких
дополнительных предположений. Так, например, чтобы получить тот же
самый результат с огрублением Больцмана, необходимо было бы
использовать дополнительное предположение, называемое "гипотезой
молекулярного хаоса" заключающейся в замене
$\rho(x_1,y_1;x_2,y_2)$ на $\rho(x_1,y_1)\rho(x_2,y_2)$ в
уравнении движения для $\rho(x,y,t)$.

\section{Эффект слабого взаимодействия}
\label{SEC4Rus}

\subsection{Малые внешние возмущения}

Рост энтропии ансамбля может быть достигнут даже без огрубления,
путем введения небольшого внешного возмущения в Преобразование
Пекаря. Возмущение должно быть достаточно небольшим, чтобы не
уничтожить рост макроскопической энтропии, но в то же самое время,
должно быть достаточно сильным, чтобы предотвратить обратные
процессы и  возвраты Пуанкаре. Для большинства таких возмущений
качественные особенности эволюции не зависят существенно от
детального вида возмущения.

Существуют два метода, которыми внешнее возмущение может быть
введено. Один метод состоит в том, чтобы ввести небольшой внешний
случайный шум. Макроскопические процессы с увеличением
макроскопической энтропии устойчивы по отношению к такому шуму.
Однако, площадь области определения функции фазовой плотности
больше не является инвариантом по отношению к возмущенному
Преобразованию Пекаря. Этим методом энтропия ансамбля может
увеличиваться.

Другой метод состоит в том, чтобы ввести слабое взаимодействие с
окружающей средой (которой может служить и "наблюдатель"). Снова,
макроскопические процессы с увеличением макроскопической энтропии
устойчивы, но площадь области определения функции фазовой
плотности больше не является инвариантом по отношению к
возмущенному Преобразованию Пекаря. Следовательно, энтропия
ансамбля может увеличиваться. Однако, такая система больше не
изолирована. Теперь она часть большей системы, разделенной на две
подсистемы. Следовательно, как было уже объяснено в Разделе
~\ref{SECcoarsRus}, огрубленная энтропия ансамбля для полной
системы может быть определена как сумма неогрубленных энтропий
множества его подсистем. В следующем подразделе мы изучим слабые
взаимодействия с окружающей средой более подробно.

\subsection{Слабое взаимодействие и дезорганизация состояния с противоположными стрелами времени подсистем}
\label{SECweakintRus}

Для дальнейшего необходимо выбрать некоторое определенное
взаимодействие между двумя "газами". В отсутствии взаимодействия,
каждый из них эволюционирует согласно Преобразованию Пекаря. Мы
помещаем два единичных квадрата один над другим и определяем
взаимодействие с максимальным расстоянием  $\sigma$ таким образом,
что, между двумя последовательными шагами Преобразования Пекаря,
все самые близкие пары частиц (с расстоянием между частицами,
меньшим чем  $\sigma$ ) обмениваются местами. (Более детально, мы
сначала находим пару самых близких частиц (с расстоянием между
частицами, меньшим чем $\sigma$ ) и обмениваем их местами. После
этого, мы находим вторую пару самых близких частиц (с расстоянием
между частицами, меньшим чем  $\sigma$ , и отличные от ранее уже
найденных частиц) и обмениваем их местами также. Мы повторяем эту
процедуру до тех пор, пока не исчерпываются все такие частицы.)
Эти взаимодействия определяются только между частицами лежащими в
различных подсистемах. Такое взаимодействие не затрагивает
движение частиц, но вызывает перемешивание между двумя
подсистемами. Обратим также внимание, что такое перемешивание не
ведет к парадоксу Гиббса, так как мы рассматриваем эти два
единичных квадрата как две различные подсистемы. Макроскопическая
энтропия определена как сумма макроскопических энтропий этих двух
подсистем.

Теперь позвольте нам рассматреть случай, в котором стрелы времени
этих двух подсистем имеют одинаковое направление. Процессы, в
которых макроскопические энтропии этих двух подсистем
увеличивается, являются устойчивыми по отношению к взаимодействию.
Таким образом, большинство низкоэнтропийных начальных условий
ведет к росту макроскопической энтропии обеих подсистем, так же
как полной системы.

Точно так же, если мы обращаем описанный выше процесс с
увеличением макроскопической энтропии, мы получаем систему, в
которой макроскопическая энтропия обеих подсистем, так же как
полной системы {\em уменьшается}. В этом смысле, взаимодействие не
разрушает симметрию между двумя направлениями времени.

Теперь позвольте нам рассмотреть самый интересный случай, в
котором энтропия увеличивается в первой подсистеме и уменьшениях
во второй. Начальное состояние первой подсистемы обладает низкой
энтропией (например, все частицы находятся в некотором небольшом
квадрате около точки  $(0,0)$ единичного квадрата). Аналогично,
вторая подсистема обладает низкой энтропией (например, все частицы
находятся в некотором небольшом квадрате около точки $(1,1)$
единичного квадрата) в  {\em конечном} состоянии.

Если бы не было никакого взаимодействия, то конечное состояние
первой подсистемы было бы высоко-энтропийным состоянием,
соответствующим почти равномерному распределению частиц.
Аналогично, начальное состояние второй системы было бы
высоко-энтропийным состоянием той же самой формы.

Однако описанные выше решения с двумя противоположными стрелами
времени больше не будут решениями, когда взаимодействие
присутствует. В большинстве случаев, взаимодействие смешивает
частицы между подсистемами. Число решений со взаимодействием,
которые имеют те же начально-конечные условия, описанные выше ,
является очень небольшим, фактически  {\em намного меньшим, чем
число таких решений в отсутствии взаимодействия.}

Позвольте сделать последнее утверждение более количественным.
После нечетного числа обменов между подсистемами частица проходит
к другой подсистеме. Аналогично, после четного числа таких
обменов, она остается в той же самой подсистеме. Вероятности для
этих двух событий равны  $p=1/2$ и не зависят от других частиц, по
крайней мере, приблизительно. Далее, мы можем утверждать, что
смешивание между этими двумя подсистемами незначительно в
начальных и конечных состояниях, поскольку энтропии этих двух
подсистем совершенно различны. Мы хотим вычислить вероятность
небольшого смешивания для конечного состояния, при условии, что
смешивание является небольшим в начальном состоянии. Для
определенности мы будем считать, что смешивание является
небольшим, если число частиц $N_t$ , перешедших из одной
подсистему в другую,  является или $N_t<N/4$, или $N_t>3N/4$. 
(Вспомним , что обмен частицами - {\em только} эффект возмущений, таким образом перемешивание не может зависеть ни от какой другой переменной, кроме $N_t$. Факторы $1/4$ и $3/4$, конечно, выбраны произвольно, но мы устанавливаем их так, чтобы получить некоторые конкретные результаты в простой итоговой форме. Качественные результаты, которые отсюда следуют, не зависят от этого конкретного выбора.)

Таким образом, вероятность дана совокупным биномиальным
распределением $F(N_t;N,1/2)$, описываемым
\begin{equation}
 F(k;n,p) = \sum_{i=0}^{\lfloor k\rfloor}
\left(
\begin{array}{l}
n \\ i
\end{array}
\right)
p^i (1-p)^{n-i}
\end{equation}
где $\lfloor k\rfloor$ является самым большим целым числом, меньше
чем или равным  $k$. Функция $F(k;n,p)$ , удовлетворяет
неравенству
\begin{equation}
 F(k;n,p) \leq \exp \left( -2\frac{(np-k)^2}{n} \right) .
\end{equation}
Состояние с  противоположными стрелами времени подсистем не
дезорганизовано, когда  $N_t<N/4$ or $N_t>3N/4$. Вероятность этого
равна
\begin{equation}
 2F(N/4;N,1/2) \leq 2e^{-N/8} .
\end{equation}
Ясно, что эта вероятность уменьшается по экспоненте с увеличением
$N$. Это означает, что такая вероятность пренебрежимо мала для
большого  $N$. Следовательно, почти бесспорно можно утверждать,
что процессы с противоположными стрелами времени будут
дезорганизованы.

В  описанной выше модели, мы нуждаемся в почти равном числе частиц
в этих двух подсистемах, чтобы дезорганизовать состояния с
противоположными стрелами времени. Это связанно с тем, что одна
частица может влиять на движение только одной близкой частицы. Для
более реалистических взаимодействий одна частица может влиять на
движение большого количества соседних частиц, что означает, что
даже очень небольшое количество частиц в одной системе может
разрушить процессы с уменьшением энтропии для другой системы.

\subsection{Декорреляция в системе с взаимодействием}

Гамильтоновы системы описываются не только макросостояниями, но
также и сложными нелинейными корреляциями между микросостояниями.
Эти корреляции ответственны за обратимость. Взаимодействие между
двумя подсистемами разрушает эти корреляции в подсистемах, но
полная система остается обратимой, то есть, корреляции появляются
в полной системе. Таким образом, декорреляция в подсистемах
распространяет корреляции на полную систему. (Этот процесс -
классический аналог декогеренции в квантовой механике).

Позвольте нам изложить эти качественные идеи в более
количественной форме. Линейная корреляция (корреляция Пирсона)
имеет поведение, очень подобное поведению нелинейных корреляций,
описанного выше. Единственная разница в том, что эти линейные
корреляции уменьшаются со временем. Взаимодействие, которое мы
предложили, может быть аппроксимировано случайным шумом с
амплитудой, соответствующей расстоянию взаимодействия между
частицами.

   Поэтому, мы ожидаем, что взаимодействие не только вызывает
выравнивание стрел времени, но также ведет к затуханию корреляций,
которое происходит даже более значительно, чем это без
взаимодействия (Раздел~\ref{SECdecorRus}). Во время этого процесса
эволюция подсистем становится необратимой, но полная система
остается обратимой.



Мы можем количественно найти величину этого затухания корреляций,
вычисляя корреляцию Пирсона для наших подсистем, описываемую
\begin{equation}
 r(m)=\frac{C(m)}{\sqrt{C(0)\langle C^m(0)\rangle}},
\end{equation}
где $\langle C^m(0)\rangle$ )> - ожидаемая дисперсия случайной
величины $x$, вычисленной после $m$ итераций отображения.
Дисперсия
 $C^m(0)$ может быть вычислена как
as
\begin{equation}
 C^m(0)=\sum_{j=0}^{2^m-1}\int\limits_{j2^{-m}}^{(j+1)2^{-m}}\left(2^mx-j-\langle
x\rangle+S\right)^2dx,
\end{equation}
где $S$ - случайное число, определенное как
$S=\sum_{k=0}^{m-1}2^k\zeta_k$. Здесь $\zeta_k$ - независимое и
однородно распределенное случайное число с нулевым средним и
дисперсией  $\sigma^2$, которое моделирует влияние взаимодействий
на эволюцию системы. После короткого вычисления мы получаем
\begin{equation}
 \langle C^m(0)\rangle=C(0)+\langle S^2\rangle=C(0)+\sum_{k,k'=0}^{m-1}2^{k+k'}\langle
\zeta_k\zeta_{k'}\rangle .
\end{equation}
Используя следующее свойство независимых и однородно
распределенных случайных величин
$\langle\zeta_k\zeta_{k'}\rangle=\delta_{kk'}\sigma^2$, мы
получаем
\begin{equation}
  \langle C^m(0)\rangle=C(0)+\frac{2^{2m}-1}{3}\sigma^2.
\end{equation}
Ясно, что взаимодействие увеличит затухание как минимум линейных
корреляций, потому что
\begin{equation}\label{eq22Rus}
 r(m)=\frac{2^{-m}}{\sqrt{1+4(2^{2m}-1)\sigma^2}}.
\end{equation}
Однако для полной системы корреляция Пирсона  $r(m)=2^{-m}$
остается той же самой. Так как $\langle S^2 \rangle^{1/2}$ должен
быть намного меньшим, чем размер системы (единичный квадрат), мы
можем заключить, что наши предположения, приводящие к
(\ref{eq22Rus}), правильны только для   $\langle S^2 \rangle =
[(2^{2m}-1)/3]\sigma^2 \ll 1$ and $ \sigma^2/2^{-2m}\ll 1$.



\subsection{Численное моделирование}
\label{SECnumsim}



Пока, мы использовали лишь общие абстрактные аргументы. В этом
подразделе мы поддержим эти аргументы конкретным численным
моделированием. Мы имеем две подсистемы (маркированные как 1 и 2),
каждая с  $N_1=N_2=300$ частиц. Эти две подсистемы занимают два
единичных квадрата. Чтобы определить огрубленную энтропию, каждый
единичный квадрат разделен на  $16\times 16 =256$ небольших
квадратов. Таким образом, энтропия каждой из этих двух подсистем
даётся
\begin{equation}
 S_{i}=-N_i \sum_{k=1}^{512} f_{k,i} \log f_{k,i},
\end{equation}
где $i=1,2$, $f_{k,i}=n_{k,i}/N_i$ и $n_{k,i}$ являются числом
частиц в соответствующих маленьких квадратах. Аналогично, полная
энтропия определяется как
\begin{equation}
 S=-(N_1+N_2)\sum_{k=1}^{512} f_{k} \log f_{k},
\end{equation}
где $f_{k}=(n_{k,1}+n_{k,2})/(N_1+N_2)$

Для системы 1 мы выбираем начальное состояние с нулевой энтропией
в  $t=1$ (см. Рис.~\ref{t=1}). Точно так же, для системы 2 мы
выбираем "конечное" состояние  с нулевой энтропией  в $t=6$..
Такие начальные условия обеспечивают, что в отсутствии
взаимодействий $S_1$ iувеличивается со временем, в то время как
$S_2$ уменьшается со временем для  $t< 6$.

Чтобы избежать численных проблем, являющихся результатом конечной
точности компьютерного представления рациональных чисел,
(\ref{eq27Rus}) заменено на  $x' = ax - \lfloor ax\rfloor$,
$y'=(y+\lfloor ax\rfloor)/2$ с $a=1.999999$. Результаты численного
моделирования представлены в Рис.~\ref{fignoint} и
Рис.~\ref{figint}.

\begin{figure*}[t]
\centerline{\includegraphics[width=8cm]{Pocetak.eps}}
% \includegraphics{figfol0}
\caption{\label{t=1} Начальнаое распределение частиц в момент $t=1$.}
\end{figure*}

\begin{figure*}[t]
\centerline{\includegraphics[width=8cm]{NoInteraction.eps}}
% \includegraphics{figfol1}
\caption{\label{fignoint}Эволюция энтропии без взаимодействия.}
\end{figure*}


Чтобы включить эффекты взаимодействия, мы определяем
взаимодействие следующим образом. (Ради вычислительного удобства
это определено немного по-другому, чем в Разделе
~\ref{SECweakintRus}.) ). 
(Взаимодействие, используемое в разделе ~\ref {SECweakint} выбрано так, чтобы сделать аналитические методы расчета более простыми, в то время как в существующей секции оно выбрано так, чтобы делать числовые вычисления более простыми.)
Мы берем небольшой диапазон
взаимодействия $r_y=0.01$ в $y$-направлении, который, по сути,
является параметром, описывающим слабость взаимодействия.
(Вспомним, что $y$ и $x$ являются аналогами канонической
координаты и канонического импульса, соответственно, в
Гамильтоновом фазовом пространстве). Взаимодействие обменивает
самые близкие пары так же как в Разделе~\ref{SECweakintRus}, но
теперь "самое близкое" относятся к расстоянию в $y$-направлении, и
нет никакого обмена, если самое близкое расстояние больше чем
$r_y$. Кроме того, теперь взаимодействие определено таким образом,
что только $x$-координаты частиц обмениваются. Выбирая те же самые
начальные условия в  $t=1$ как в случае отсутствия
взаимозависимости (Рис.~\ref{t=1}), результаты численного
моделирования с взаимодействием представлены на
Рис.~\ref{figint}. Мы видим, что с взаимодействием
(Рис.~\ref{figint}) $S_2$ S2 начинает увеличиваться в более
раннее время, чем без взаимодействия (Рис.~\ref{fignoint}).


\begin{figure*}[t]
\centerline{\includegraphics[width=8cm]{Interaction.eps}}
% \includegraphics{figfol2}
\caption{\label{figint} Эволюция энтропии при взаимодействии.}
\end{figure*}




\begin{figure*}[t]
\centerline{\includegraphics[width=8cm]{Symmetric_inter.eps}}
\caption{\label{figintsym} Симметричная эволюция энтропии при взаимодействии.}
\end{figure*}

Наконец, мы даем пример симметричного развития времени при взаимодействии.
 Для этой цели, мы выбираем нулевую энтропию начального состояния в $t=0$ и для системы 1 и для системы 2. 
Два начальных распределения частиц (для двух подсистем) при нулевой энтропией различны. 
В частности они расположены в пределах двух различных маленьких квадратов, 
так что полная начальная энтропия  больше, чем ноль. Результат числового моделирования представлен 
на Рис. ~\ref {figintsym}. Мы видим, что решение является симметричным при инверсии времени $t \rightarrow - t$.



\section{Выводы}
\label{SEC5Rus}

В этой статье мы использовали "игрушечную" модель, основанную на
Преобразовании Пекаря, чтобы продемонстрировать особенности,
которые, справедливы для общих систем, описанных обратимой
Гамильтоновой механикой. Ясно, для таких систем можно свободно
выбрать или конечные, или начальные условия, но нельзя свободно
выбрать смешанные начально-конечных условия. Начально-конечных
условия - это условия, при которых канонические параметры для
одной части частиц определены в начальный момент времени, а для
другой части - в конечный момент. Для многих смешанных
начально-конечных условий не существует соответствующего решения
(для Гамильтоновых уравнений движения). Точно так же, как для
нашей "игрушечной модели", для большинства Гамильтонианов со
слабыми взаимодействием, число решений с данными крупнозернистыми
начально-конечными условиями намного меньше, чем число решений с
только крупнозернистыми начальными условиями, или только
крупнозернистыми конечными условиями. Это объясняет, почему,
практически, мы никогда не наблюдаем подсистемы с противоположными
стрелами времени, то есть, почему стрела времени универсальна.

В некотором смысле, дезорганизация состояний с  противоположными
стрелами времени подобна эргодичности. Оба свойства справедливы во
всех практических ситуациях, однако они не являются точными
законами. Они верны для большинства реальных систем, но
контр-примеры могут всегда быть найдены
\cite{schul1,schul2}. Кроме того, оба свойства кажутся
интуитивно очевидными, но доказать их строго очень трудно. Для
эргодичности соответствующим строгим результатом  является KAM
(Колмогоров-Арнольд-Мозер) теорема, в то время как для
дезорганизации состояний с противоположными стрелами времени такая
строгая теорема отсутствует.

Наши результаты также разрешают "противоречие" между "Новой
Динамикой" Пригожина \cite{prigogine1} (обсужденной в Разделе
~\ref{SECcoarsRus} из данной работы) и комментарием Bricmont
\cite{bricmont}. Динамика взаимодействующих подсистем может
быть разделена на два типа динамик:
\begin{enumerate}
\item Обратимую {\em идеальную динамику}, рассматриваемую
относительно координатного времени, когда энтропия может или
уменьшиться или увеличиться.
 \item Необратимую {\em наблюдаемую динамику}, рассматриваемую  относительно характерных
 стрел времени взаимодействующих подсистем,
 относительно которых энтропия может только увеличиваться, как уже показано выше.
\end{enumerate}
В рамках этой терминологии "Новая Динамика" Пригожина
\cite{prigogine1} является одной из форм {\em наблюдаемой
динамики}, в то время как статья Bricmont  \cite{bricmont}
рассматривает {\em идеальную динамику}. В частности, наблюдаемая
динамика не включает возвращения Пуанкаре и обратимость, которые
являются действительно ненаблюдаемыми реальным наблюдателем. Это
делает её более простой, чем идеальная динамика. Однако, в
принципе, оба типа динамики правильны.

Это рассуждение может также быть применено к интерпретации числовых результатов в Разделе. ~\ref {SECnumsim}. Как Рис. ~\ref {fignoint}, так и рис. ~\ref {figint} показывают, что стрела времени, определенная полной энтропией, полностью обращается в некоторый момент времени. Это обращение соответствует описанию идеальной динамикой. Но может ли быть наблюдаемо такое обращение? Ради концептуальной ясности мы подчеркиваем, что наблюдатель - только одна из подсистем, и разделяем вопрос на три различных. Первое,  может ли наблюдатель наблюдать обращение  своей {\em собственный} стрелы времени? Во- вторых, наблюдатель может наблюдать обращение стрелы времени  {\em его полного окружения}? Третье,  может ли наблюдатель наблюдать обращение стрелы времени {\em малой части}  окружающей его среды? 

Ответ на первый вопрос - {\em нет}, потому что наблюдатель естественным образом определяет стрелу времени как направление, в котором его собственная энтропия увеличивается. А именно, наблюдатель чувствует субъективный опыт потока времени, потому что каждый раз он имеет доступ к его памяти о некоторых событиях, которые не случаются прямо сейчас. Такие события естественно интерпретируются как его "прошлое". Можно утверждать, что память может работать, только когда энтропия увеличивается в направлении от запоминаемого случая до времени вспминания его (см., например, \cite {nik1}). Точно так же другие процессы в мозгу (или компьютере) также, кажется, требуют увеличения энтропии для их нормального  функционирования (см. также \cite{penrose}). Таким образом, ожидается, что субъективный опыт наблюдателя о потоке времени всегда совпадает с направлением, в котором энтропия наблюдателя увеличивается. 

Ответ на второй вопрос - {\em почти наверняка нет}, потому что, если полная окружение наблюдается, тогда оно взаимодействует с наблюдателем, и, следовательно, их стрелы времени имеют тенденцию быть сонаправлены, кроме, возможно,  очень короткого времени, необходимого для процесса выравнивания направлений.

Ответ на третий вопрос  {\em иногда да, но обычно нет}. А именно, некоторые специальные системы (например, спин-эхо, обсуждаемое в Разлеле. ~\ref {SEC2})
 может слабо взаимодействовать с их окружающей средой и все еще сохранить стрелу времени противонаправленной окружающей среде относительно долгое время. 
Такие специальные системы - относительно маленькие части полной окружающей среды, 
и наблюдатель может заметить, что такая подсистема имеет стрелу времени противоположную стреле времени этого наблюдателя.
 Действительно, поскольку мы уже объяснили в Разделе. ~\ref{SEC2Rus}, наши результаты, основанные на вероятностных рассуждениях 
для большинства система и не подразумевают, что абсолютно невозможно наблюдать подсистему, в которой энтропия уменьшается. 
Они только объясняют, почему такие системы, как ожидается, будут очень редкими, что соответствует нашему каждодневному опыту.



Тесно связанное с вышеизложенным наблюдение - это то, что наши результаты не находятся в противоречии с существованием диссипативных систем
\cite{prigogine2} (таких как, например, определенные
самоорганизующиеся биологические системы), в котором энтропия
подсистемы может уменьшиться со временем, несмотря на то, что
энтропия окружающей среды увеличивается. Энтропия полной системы
(включающей как энтропию диссипативной системы, так и окружающей
среды) увеличивается, что отвечает закону  увеличения энтропии.
Для таких систем типично, что взаимодействие с окружающей средой
{\em сильно}, в то время как результаты нашей статьи обращаются к
 {\em слабым} взаимодействиям между подсистемами. Например, для существования
  живых организмов, необходим большой поток энергии от Солнца.
  Небольшой поток энергии от звезд не достаточен для жизни, но достаточен
  для декорреляции и для выравнивания стрел времени. В работе  \cite{mac}:
приводится цитата: " Однако, наблюдатель является макроскопическим
по определению, и все отдаленно взаимодействующие макроскопические
системы становятся коррелированными очень быстро (например, Borel
замечательно вычислил, что, перемещение одного грамма материала по
звезде Сириус на один метр может влиять на траектории частиц в
газе на Земле на временных масштабах порядка микросекунд
\cite{borel})."





\section*{Благодарности}

Мы благодарим анонимного рецензента за различные идеи, позволившие улучшить качество и ясность изложения.
Работы H.N. и V.Z. были поддержаны Министерством Науки республики
Хорватии согласно Контрактам Номер 098-0982930-2864 и
098-0352828-2863, соответственно.

\appendix
\section*{Приложение}
\section{Основные свойства Преобразования Пекаря}
\label{app1Rus}

В этом приложении мы представляем некоторые основные свойства
Преобразования Пекаря. Больше деталей может быть найдено,
например, в \cite{driebe}.

\subsection{Определение Преобразования Пекаря}

Рассмотрим бинарную символическую последовательность.
\begin{equation}
 \ldots S_{-2}, S_{-1}, S_0; S_1, S_2, S_3 \ldots
\end{equation}
бесконечную с обеих сторон. Такая последовательность определяет
два вещественных числа
\begin{equation}
 x=0. S_1 S_2 S_3 \ldots , \;\;\;\;\; y=0. S_0 S_{-1} S_{-2} \ldots .
\end{equation}
Последовательность может быть перемещена обратимо относительно
точки с запятой в обоих направлениях. После левого сдвига мы
получаем новые действительные числа
\begin{equation}\label{eq27Rus}
 x' = 2x - \lfloor 2x\rfloor , \;\;\;\;\; y'=\frac{1}{2} (y+\lfloor 2x\rfloor) ,
\end{equation}
где $\lfloor x\rfloor$ является самым большим целым числом, меньше
чем или равным x. Это отображение единичного квадрата в себя
называют {\em Преобразованием Пекаря}.

У Преобразования Пекаря есть есть простая геометрическая
интерпретация, представленная в  Рис.~\ref{fig1Rus}. Там (a) -
начальная конфигурация, и (c) заключительная конфигурация после
одной итерации  Преобразования Пекаря, с промежуточным шагом,
представленным в (b). Часть (d)  представляет заключительную
конфигурацию после двух итераций.

\begin{figure*}[t]
\centerline{\includegraphics[width=15cm]{baker1.eps}}
% \includegraphics{figfol1}
\caption{\label{fig1Rus}Геометрическая интерпретация
Преобразования Пекаря. (a) Начальная конфигурация (b) Однородное
сжатие в вертикальном направлении и расширение в горизонтальном
направлении на величину фактора 2 (c) Итоговая конфигурация после
отрезания правой половины и её помещения на левую (d) Итоговое
конфигурация после двух итераций.}
\end{figure*}

\subsection{Нестабильные периодические орбиты}

Периодические символические последовательности  $(0)$ и $(1)$
соответствуют неподвижным точкам $(x,y)=(0,0)$ и $(x,y)=(1,1)$),
соответственно. Периодическая последовательность  $(10)$
соответствует двухпериодичной орбите  $\{ (1/3,2/3), (2/3,1/3)\}$.
Из периодической последовательности $\ldots 001;001 \ldots$ мы
получаем  $\{(1/7,4/7), (2/7,2/7), (4/7,1/7) \}$. Точно так же из
$\ldots 011;011 \ldots$ мы получаем $\{(3/7,6/7), (6/7,3/7),
(5/7,5/7) \}$.

Любой $x$ и $y$ могут быть аппроксимированы произвольно хорошо
 $0.X_0\ldots X_n$ и $0.Y_0\ldots Y_m$, соответственно, при условии, что $n$ и $m$
 являются достаточно большими. Поэтому периодическая последовательность
$(Y_m\ldots Y_0 X_0\ldots X_n)$, может приблизиться к любой точке
единичного квадрата произвольно близко. Таким образом, множество
всех периодических орбит даёт плотное множество на единичном
квадрате.


\subsection{Эргодичность, перемешивание, и сохранение площади}

Из-за растяжения в горизонтальном направлении, все близкие точки
расходятся по экспоненте под действием итераций  Преобразования
Пекаря. При этих итерациях любая случайная символическая
последовательность приближается произвольно  близко к любой точке
единичного квадрата. Вообще, такое эргодическое свойство может
использоваться, чтобы заменить среднее по "времени"  $\langle
A\rangle$ средним по "ансамблю"
\begin{equation}
\langle A \rangle = \sum_n A(x_n,y_n) = \int A(x,y) \, d\mu(x,y) =
\int A(x,y) \rho(x,y) \, dx \, dy,
\end{equation}
где $d\mu(x,y)$ является инвариантной мерой и  $\rho(x,y)$
инвариантная плотность для Преобразования Пекаря. Для
Преобразования Пекаря,  $\rho(x,y)=1$.

Под действием итераций Преобразования Пекаря любая область
отображается в ряд узких горизонтальных полос. В конечном счете,
они заполняют равномерно весь единичный квадрат, что и
соответствует перемешиванию. Точно так же обратные итерации
отображают область в узкие вертикальные ленты, которая также
соответствует перемешиванию.

Во время этих итераций не изменяется площадь область. Это свойство
- закон сохранения площади области для Преобразования Пекаря.

\subsection{Показатели степени Ляпунова, сжимающиеся и растягивающиеся направления}

Если $x_0^{(1)}$ и $x_0^{(2)}$ имеют равные первые  $k$ двоичные
цифры, то для  for $n<k$,
\begin{equation}
 x_n^{(2)}-x_n^{(1)}=2^n (x_0^{(2)}-x_0^{(1)})
= (x_0^{(2)}-x_0^{(1)}) e^{n\log 2} ,
\end{equation}
где $\Lambda = \log 2$ iявляется первым положительным показателем
степени Ляпунова для Преобразования Пекаря. Следовательно,
расстояние между двумя близкими орбитами увеличивается по
экспоненте с увеличением  $n$, и после $k$ iитерации становится
порядка $1$. Это свойство называют чувствительностью к начальным
условиям. Из-за этого свойства, все периодические орбиты
неустойчивы.

Так как площадь область сохраняется, растяжение в горизонтальном
направлении, обсужденная выше, подразумевает, что некоторое
направление сжатия также должно существовать. Действительно,
эволюция в вертикальном направлении  $y$ обратна эволюции в
горизонтальном направлении. Если $(x_0^{(1)},y_0^{(1)})$ и
$(x_0^{(2)},y_0^{(2)})$ являются двумя точками с
$x_0^{(1)}=x_0^{(2)}$, тогда
\begin{equation}
 y_n^{(2)}-y_n^{(1)}=2^{-n} (y_0^{(2)}-y_0^{(1)})
= (y_0^{(2)}-y_0^{(1)}) e^{n(-\log 2)} .
\end{equation}
Следовательно, $\Lambda = -\log 2$ 2 - это второй отрицательный
показатель степени Ляпунова для Преобразования Пекаря.

\subsection{Затухание корреляций}
\label{SECdecorRus}

Так как $x$- неустойчивое направление, эволюция в этом направлении
приводит к затуханию корреляций. Средняя корреляционная функция
$C(m)$ для последовательности  $x_k$ обычно определяется как
\begin{equation}
 C(m)=\lim \limits_{n \to
\infty}\frac{1}{n}\sum_{k=1}^n\left(x_k-\langle x\rangle\right) \left(x_{k+m}-\langle
x\rangle\right),
\end{equation}
где $\langle x\rangle=\lim \limits_{n \to\infty}\sum_{k=1}^n
x_k/n$. Корреляции могут быть более легко вычислены, если известна
инвариантная мера $\mu(x)$, в этом случае
\begin{equation}
 C(m)=\int\left(x-\langle x\rangle\right)\left(f^m(x)-\langle x\rangle\right)d\mu(x),
\end{equation}
где $f^m(x)=x_m$ - функция, которая отображает переменную $x$ на
ее образ после $m$ итераций Преобразования Пекаря. Для
Преобразования Пекаря $d\mu(x)=dx$, таким образом, мы можем
написать
\begin{equation}
 C(m)=\sum_{j=0}^{2^m-1}\int_{j2^{-m}}^{(j+1)2^{-m}}\left(x-\langle
x\rangle\right)\left(2^mx-j-\langle
x\rangle\right)dx,
\end{equation}
который приводит к
\begin{equation}
C(m)=\sum_{j=0}^{2^m-1}\left[2^m\frac{x^3}{3}-\left(2^m\langle
x\rangle+\langle
x\rangle\right)\frac{x^2}{2}+\langle
x\rangle^2x-j\left(\frac{x^2}{2}-\langle
x\rangle x\right)\right]_{j2^{-m}}^{(j+1)2^{-m}}.
\end{equation}
Для Преобразования Пекаря   $\langle x\rangle=1/2$, и, таким
образом, написанная выше сумма может быть вычислена явно
\begin{equation}
 C(m)=\frac{2^{-m}}{12}.
\end{equation}
Это показывает, что затухание корреляций происходит по экспоненте
с увеличением m. Корреляция Пирсона для системы находится
следующим образом
\begin{equation}
 r(m)=C(m)/C(0)=2^{-m}.
\end{equation}











\begin{thebibliography}{99}

\bibitem{reichenbach}
H. Reichenbach, {\it The Direction of Time} (University of California Press,
Los Angeles, 1971).

\bibitem{davies}
P.C.W. Davies, {\it The Physics of Time Asymmetry} (Surrey University Press, London, 1974).

\bibitem{penrose}
R. Penrose, {\it The Emperor's New Mind} (Oxford University Press, 1989).

\bibitem{price}
H. Price, {\it Time's Arrow and Archimedes' Point}
(Oxford University Press, New York, 1996).

\bibitem{zeh}
H.D. Zeh, {\it The Physical Basis of the Direction of Time} (Springer, Heidelberg, 2007).

%\bibitem{lebowitz}
%J.L. Lebowitz, arXiv:0709.0724.

\bibitem{mac}
L. Maccone, Phys. Rev. Lett. {\bf 103}, 080401 (2009).

\bibitem{vaidman}
L. Vaidman, quant-ph/9609006.

\bibitem{kuper04}
O. Kupervasser, nlin/0407033.
\bibitem{kuper05}
O. Kupervasser, nlin/0508025.

\bibitem{com1}
D. Jennings, T. Rudolph, Phys. Rev. Lett. {\bf 104}, 148901 (2010).

\bibitem{com2}
O. Kupervasser, D. Laikov, arXiv:0911.2610.

\bibitem{com3}
H. Nikoli\'c, arXiv:0912.1947.

\bibitem{mac2}
L. Maccone, arXiv:0912.5394.

\bibitem{zeh1}
H.D. Zeh, Entropy {\bf 7}, 199 (2005).
\bibitem{zeh2}
H.D. Zeh, Entropy {\bf 8}, 44 (2006).

\bibitem{kupervasser-big}
O. Kupervasser, arXiv:0911.2076.

\bibitem{thomson}
W. Thomson, Proc. Roy. Soc. Edinburgh {\bf 8}, 325 (1874); 
reprinted in S.G. Brush, {\it Kinetic Theory} (Pergamon, Oxford, 1966).

\bibitem{Leb}
J.L. Lebowitz, 
%Microscopic Reversibility and Macroscopic
%Behavior: Physical Explanations and Mathematical Derivations.
Turkish Journal of Physics {\bf 19}, 1 (1995);
%Also in 25
%Years of Non-Equilibrium Statistical Mechanics, Proceedings of
%Sitges Conference, Barcelona, Spain (1994); in Lecture Notes in
%Physics, J.J. Brey, J. Marro, J.M. Rubi and M. San Miguel (eds.),
%Springer, (1995) Texas PP. 96-163; Los Alamos 
cond-mat/9605183.

\bibitem{ellis}
G.F.R. Ellis, Gen. Rel. Grav. {\bf 38}, 1797 (2006).

\bibitem{nik1}
H. Nikoli\'c, Found. Phys. Lett. {\bf 19}, 259 (2006).

\bibitem{nik2}
H. Nikoli\'c,
\verb+http://www.fqxi.org/data/essay-contest-files/Nikolic_FQXi_time.pdf+.

\bibitem{prigogine1}
I. Prigogine, {\it From Being to Becoming}
(W.H. Freeman and Company, New York, 1980)


\bibitem{elskens}
Y. Elskens, R. Kapral, J. Stat. Phys. {\bf 38}, 1027 (1985).

\bibitem{gaspard}
P. Gaspard, J. Stat. Phys. {\bf 68}, 673 (1992).

\bibitem{hartmann}
G.C. Hartmann, G. Radons, H.H. Diebner, O.E. Rossler,
Discrete Dynamics in Nature and Society {\bf 5}, 107 (2000).

\bibitem{schul1}
L.S. Schulman, Phys. Rev. Lett. {\bf 83}, 5419 (1999).
\bibitem{schul2}
L.S. Schulman, Entropy {\bf 7}, 208 (2005).



\bibitem{bricmont}
J. Bricmont, chao-dyn/9603009.

\bibitem{prigogine2}
I. Prigogine, {\it Self-organization in nonequilibrium systems}
(John Wiley \& Sons, 1977).

\bibitem{borel}
E. Borel, {\it Le Hasard} (Alcan, Paris, 1914).

\bibitem{driebe}
D.J. Driebe, {\it Fully Chaotic Maps and Broken Time Symmetry}
(Kluwer Academic Publishers, Dordrecht, 1999).















\end{thebibliography}




